S-BDT: Distributed Differentially Private Boosted Decision Trees

We introduce S-BDT: a novel $(\varepsilon,\delta)$-differentially private distributed gradient boosted decision tree (GBDT) learner that improves the protection of single training data points (privacy) while achieving meaningful learning goals, such as accuracy or regression error (utility). S-BDT uses less noise by relying on non-spherical multivariate Gaussian noise, for which we show tight subsampling bounds for privacy amplification and incorporate that into a R\'enyi filter for individual privacy accounting. We experimentally reach the same utility while saving $50\%$ in terms of epsilon for $\varepsilon \le 0.5$ on the Abalone regression dataset (dataset size $\approx 4K$), saving $30\%$ in terms of epsilon for $\varepsilon \le 0.08$ for the Adult classification dataset (dataset size $\approx 50K$), and saving $30\%$ in terms of epsilon for $\varepsilon\leq0.03$ for the Spambase classification dataset (dataset size $\approx 5K$). Moreover, we show that for situations where a GBDT is learning a stream of data that originates from different subpopulations (non-IID), S-BDT improves the saving of epsilon even further.

==> related_work.tex <==
Our work concentrates on GBDTs as a data-frugal ML technique, which does not need a large amount of data for strong utility-privacy tradeoffs.
%
Prior work on learning decision tree ensembles in DP includes an algorithm by Bojarski et al.~\cite{bojarski2014differentially} to learn random forests in DP and a work by Li et al.~\cite{li2020privacy} to learn gradient boosted decision tree ensembles in DP.

The work by Bojarski et al.~\cite{bojarski2014differentially} proposes to use many random splits instead of learning a few good splits. That work proves utility bounds for randomly choosing splits, yet does not utilize the potential of gradient boosted ensemble learning, subsampling and individual Rényi filters.

Closest to our results is the work by Li et al.~\cite{li2020privacy} for learning gradient boosted decision tree ensembles (GBDT) in a differentially private manner. We give an overview over their algorithm in ~\Cref{sec:dpboost_overview}. Li et al. propose to use the exponential mechanism for finding strong splits and introduce a novel technique, called gradient-based data filtering. Gradient-based data filtering filters out data points with large gradients and leaves them for later trees, hoping that these points will have a smaller gradient when training later trees.
We experimentally show, however, that their gradient-based data filtering does not provide any improvement. Further, their work does not use a differentially private initial score, which can improve GBDT learning, it does not utilize privacy amplification methods, and has a leaf noise scale that does not decrease with the number of data points. As a result, we do not consider the work of Li et al. to be data-frugal.

Other data-frugal learners are SVMs or other ML techniques with convex optimization techniques. They also  achieve strong utility-privacy tradeoffs with few data points~\cite{ChMoSa_11:dperm}. Yet, compared to convex learners, GBDTs are able to learn highly non-linear problems.
